EffectWAM: Learning Action-Grounded Effects for Robot Manipulation

World-action models connect visual prediction with executable robot control. We present EffectWAM, which develops this connection through three complementary components: Effect, camera positional encoding (CaPE), and Action Grounding. Effect represents visual change as the difference between independently encoded future observations and a shared current-observation anchor. CaPE conditions endpoint pooling on relative camera pose when reliable extrinsics are available, while sharing the same learned parameters with pose-free pooling for uncalibrated trajectories. Action Grounding trains the visual representation to retain measured changes in end-effector pose and gripper state. An exponential moving average of the observation encoder supplies Effect targets. A shared generation expert learns to jointly predict Effect and an executable action chunk through flow matching, and reuses the sampled pair to generate future video on demand. This allows the controller to execute actions without waiting for video synthesis. We train on more than 20,000 hours of heterogeneous embodied data, excluding unused chain-of-thought data, and accommodate dataset-specific joint, end-effector, and hand-pose representations. Our evaluation uses the Small (8B) configuration on all five benchmarks and additionally evaluates the Large (26B) configuration on RoboDojo. Experiments examine closed-loop manipulation across complementary benchmarks, and comparisons across multiple baseline policies show consistent improvements from Action Grounding.

==> iFlyBot_sections/overview.tex <==
\section{Overview}
\label{sec:system_overview}

\textbf{EffectWAM} connects language-conditioned robot control with prediction of the visual changes accompanying an action. The framework centers on three components: Effect, CaPE, and Action Grounding. The generation modules jointly predict an Effect sequence and an executable action chunk, then optionally reuse this pair to generate a future video. The architecture and objectives are detailed in Sec.~\ref{sect:model}.

\paragraph{Effect and joint generation.}
A shared observation encoder processes current and future frames independently. Differences from the current endpoint form compact Effect targets, maintained through an exponential moving average encoder. A trainable ViT supplies visual features to the semantic expert, while a frozen VAE supplies the observed visual latent. The action-generation pathway uses this context and the task instruction to sample Effect and actions jointly. The video-generation pathway optionally forecasts future frames conditioned on the same sampled pair.

\paragraph{CaPE and Action Grounding.}
CaPE conditions endpoint pooling on camera pose relative to the current frame when reliable calibration is available. The pose-free route shares the same learned weights. Action Grounding supervises the endpoint differences with measured changes in end-effector pose and gripper state, retaining quantities relevant to control while masking unavailable measurements. These components address complementary aspects of learning visual transitions: viewpoint variation and physical motion.

\paragraph{Heterogeneous data and model scale.}
The training corpus contains more than 20,000 hours of embodied data, excluding unused chain-of-thought data. Dataset-specific interfaces preserve joint, end-effector, and hand-pose semantics when constructing action targets. All five benchmarks are evaluated with Small (8B), and RoboDojo is additionally evaluated with Large (26B). Results for the two scales are identified separately.

